Digital Gatekeepers: Google's Role in Curating Hashtags and Subreddits

Search engines play a crucial role as digital gatekeepers, shaping the visibility of Web and social media content through algorithmic curation. This study investigates how search engines like Google selectively promotes or suppresses certain hashtags and subreddits, impacting the information users encounter. By comparing search engine results with nonsampled data from Reddit and Twitter/X, we reveal systematic biases in content visibility. Google's algorithms tend to suppress subreddits and hashtags related to sexually explicit material, conspiracy theories, advertisements, and cryptocurrencies, while promoting content associated with higher engagement. These findings suggest that Google's gatekeeping practices influence public discourse by curating the social media narratives available to users.

==> images/twitter_toxic_binary.tex <==

\begin{tikzpicture}
    \begin{axis}[
        height=5cm,
        width=8cm,
        ymin=0,
        ymax=1,
        xlabel={},
        ylabel={Probability},
        xtick={1, 2, 3},
        xticklabels={Not in SERP, In SERP, Ret. By SERP},
        x tick label style={rotate=45, anchor=east, font=\scriptsize},
        enlarge x limits=0.2, % Adjusting space for bars
        bar width=0.3, % Adjusted bar width
        legend style={at={(0.5,-0.15)}, anchor=north, legend columns=2}, % Positioning the legend below
        title={Twitter/X},
    ]
        % Neutral Data
        \addplot+[
            ybar,
            draw=blue,
            pattern=horizontal lines, % Add horizontal lines pattern
            pattern color=blue, % Adjust the pattern color
            error bars/.cd,
            y dir=both,
            y explicit,
            error bar style={black},
        ] coordinates {
            (1-0.15, 0.9471683009933332) +- (0, 0.013389219461309713) % Not in SERP, Neutral
            (2-0.15, 0.9065520586121129) +- (0, 0.017665846390597015) % In SERP, Neutral
            (3-0.15, 0.9367880400174763) +- (0, 0.01472336912739181) % Ret. By SERP, Neutral
        };

        % Toxic Data
        \addplot+[
            ybar,
            draw=red,
            pattern=dots, % Add dots pattern
            pattern color=red, % Adjust the pattern color
            error bars/.cd,
            y dir=both,
            y explicit,
            error bar style={black},
        ] coordinates {
            (1+0.15, 0.052831696592791556) +- (0, 0.013389219656041316) % Not in SERP, Toxic
            (2+0.15, 0.09344793654930982) +- (0, 0.01766584641791572) % In SERP, Toxic
            (3+0.15, 0.06321195671356326) +- (0, 0.014723369324086386) % Ret. By SERP, Toxic
        };

        % Add legend entries
        \legend{Neutral, Toxic}
    \end{axis}
\end{tikzpicture}

